An Empirical Study on Ethereum Private Transactions and the Security Implications

Recently, Decentralized Finance (DeFi) platforms on Ethereum are booming, and numerous traders are trying to capitalize on the opportunity for maximizing their benefits by launching front-running attacks and extracting Miner Extractable Values (MEVs) based on information in the public mempool. To protect end users from being harmed and hide transactions from the mempool, private transactions, a special type of transactions that are sent directly to miners, were invented. Private transactions have a high probability of being packed to the front positions of a block and being added to the blockchain by the target miner, without going through the public mempool, thus reducing the risk of being attacked by malicious entities. Despite the good intention of inventing private transactions, due to their stealthy nature, private transactions have also been used by attackers to launch attacks, which has a negative impact on the Ethereum ecosystem. However, existing works only touch upon private transactions as by-products when studying MEV, while a systematic study on private transactions is still missing. To fill this gap and paint a complete picture of private transactions, we take the first step towards investigating the private transactions on Ethereum. In particular, we collect large-scale private transaction datasets and perform analysis on their characteristics, transaction costs and miner profits, as well as security impacts. This work provides deep insights on different aspects of private transactions.

==> 4-eval.tex <==
\section{Analysis on Private Transactions}
\label{sec:eval}

In this section, we describe the overall statistics of \pri \txs by answering the following four questions. Each question is related to one subsection. Besides, the first three questions relate to our G1 and the fourth question is for G2 in ~\secref{sec:sys:goal}.
\begin{packeditemize}
    \item \textbf{Q1: How popular are \pri \txs?} In particular, what is the distribution of \pri \txs inside and outside blocks? Besides, what are the features of \pri \txs from used gas and gas limit from blocks?
    \item \textbf{Q2: What are the purposes of private transactions?} Specifically, what are the types of \pri \txs and they used for? 
    \item \textbf{Q3: What kinds of tokens and DeFi platforms are mostly used in the private transactions?}
    \item \textbf{Q4: What are the results of arbitrage detection in \pri \txs?}
\end{packeditemize}

\subsection{Characteristics}
\subsubsection {The count and percentage of \pri \txs per month.} 
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/411ptxs/411_count_rate_of_px.pdf}
    \caption{The count and percentage of private transactions per month(x1: \pri \txs per month, x2:percentage in total \txs per month; y: count).} 
    \hfill
    \label{figs:txnum}
    \end{figure}
    
    First and foremost, we measure the count of \pri \txs against per month.
    As shown in ~\figref{figs:txnum}, there are at least 0.28 million \pri \txs every month and around 0.60 million \pri \txs on average per month. 
    Besides, the percentage of \pri \txs among all the \txs account for 2\% on average per month. 
    Overall, there are not many \pri \txs in the total mined \txs, while the percentage of \pri \txs mostly keeps increasing slightly every month. 
    
    \lesson{The count of \pri \txs keeps slightly increasing over month.}


\subsubsection{The distribution of \pri \txs within blocks.}
\label{sec:char:dis}
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/412ptxs/block_px_count_and_peak1.pdf}
    \caption{The count of \pri \txs per block(x:block number ; y: the of count of \pri \txs in a block).} 
    \label{figs:pritxperblock}
    \end{figure}
    
    
    % \begin{figure}[t]
    % \centering
    % \includegraphics[width=1\columnwidth]{figs/412ptxs/412_rate_of_px_range.pdf}
    % \caption{The percentage of blocks by the count of \pri \txs within one block(x: the percentage of blocks in this range; y: the range of count of \pri \txs in a block).} 
    % \label{figs:rate_pritxperblock}
    % \end{figure}
    
    We observe 1,259,251 blocks and show the count of \pri \txs against per block in ~\figref{figs:pritxperblock}. 
    In particular, the block number starts from 12,344,945 and ends with 14,688,626. 
    Specifically, there is a block 13,440,128 who has more \pri \txs than others. 
    After a closer examination, the block 13,440,128 contains 615 private transactions, of which more than 580 are miner transfers to the EOA address.
    In addition, most of the blocks have only a few \pri \txs. 
    According to ~\figref{figs:rate_pritxperblock}, 93.2\% have less than 10 \txs within each block and 0.09\% of the blocks have more than 100 \pri \txs.

   \lesson{Most(93.2\%) of the blocks have \pri \txs contain less than 10 \pri \txs.}
 
    \bheading{Abnormal count of \pri \txs in some blocks.}
    % \begin{figure}[t]
    % \centering
    % \includegraphics[width=1\columnwidth]{figs/412ptxs/412_peak_of_px_per_block.pdf}
    % \caption{The count of \pri \txs in peak slot within one block(x: the count of blocks in this range; y: the range of count of \pri \txs in a block).} 
    % \label{figs:abnoraml}
    % \end{figure}
    We analyze the blocks in the peek periods, as shown in ~\figref{figs:pritxperblock}. There are four ranges of blocks that seem to have far more \pri \txs than other blocks. The block ranges are [13,404,461 - 13,497,355],[13,926,965 - 13,949,430], [14,057,403 - 14,133,216] and [14,636,264 - 14,664,418], respectively. ~\figref{figs:abnoraml} displays the details of the count against per block. We observe that not all of the blocks have far more \pri \txs than others and some blocks have the count of \pri \txs below the average. In particular, we study the blocks have more \pri \txs than others and have found that many \pri \txs are used for miners transferring \textit{ETH} to EOAs. \xz{maybe focus on the biggest peak and study it in depth, then mention others briefly}
    
    \lesson{There are four peek ranges where blocks mine more \pri \txs than average and these \pri \txs are mostly used for transferring money from miners.}

    \bheading{The positions of \pri \txs inside blocks.}
    \Pri \txs are usually bundled together to miners and placed at the top of the block. With the data from all the 1,259,251 blocks, we observe that all the \pri \txs are located in front of normal \txs in blocks. The results are expected since \pri \txs are created to race for the opportunities before other \txs. Thus, they should be put in the top positions of the blocks.  
    
    \lesson{\Pri \txs are placed in front of other normal \txs in blocks.}



\subsubsection{The used gas of \pri \txs.}  
    % We present the gasfee of \pri \txs, including the usedgas and gasprice.
    We present the used gas of the \pri \txs, which is the total cost of the EVM operations of \txs. Specifically, a block has gas limit to constrain the number of mined \txs. Thus, the sum of the used gas of all the \txs in a block cannot exceed the gas limit of the block. 
    \xz{we seem to focus on gas and gas fees (are they different?) a lot; why is that?}
    % Specifically, the gas limit of a block reflects how many transactions can be packaged in a single block, and the gas used can . These parameters help to analyze the activities of private transactions. \mz{@all, should this be put into the background?}
    
    \bheading{The gas limit of blocks containing \pri \txs.} 
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/413ptxs/413_gaslimit_blocks.pdf}
    \caption{The gas limit(\textit{GWei}) of blocks that have \pri \txs(x: the gas limit in \textit{GWei}; y: the number of blocks that have \pri \txs).} 
    \label{figs:glperblock}
    \end{figure}
    In ~\figref{figs:glperblock}, \xz{seem to be exactly the same as the EIP-1559 paper. Also, what is the connection between the gas limit and private tx?} we present the gas limit against per block. Before block 12,965,000, the gas limit is around 15,000,000 \textit{GWei}. Then beginning with the block 12,965,000, the gas limit is doubled to be 30,000,000 \textit{GWei}.
    The reason is that Ethereum has more \txs to deal with and the increased gas limit helps to avoid network congestion. 
    Besides, the increased gas limit of blocks explains the abnormal high count of \pri \txs in~\secref{sec:char:dis}. 
    
    \lesson{The gas limit of blocks is doubled to be 30,000,000 \textit{GWei} since block 12,965,000.}
    

    \bheading{The used gas of \pri \txs.} 
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/413ptxs/413_gasused_px.pdf}
    \caption{The used gas by \pri \txs per block(x: used gas in a block (\textit{GWei}); y: block number).}
    \label{figs:usedgas}
    \end{figure}
    ~\figref{figs:usedgas} presents the used gas of \pri \txs against per block. 
    The total used gas by \pri \txs in each block is about 780,000 \textit{GWei} on average, which accounts for 5.8\% among the total used gas.
    Particularly, there are some blocks where the used gas of \pri \txs takes a large portion of the total used gas. 
    It is obvious that \txs in such blocks are mostly \pri \txs.
    For example, the blocks starting from 13,403,072 to 13,497,355 have a high percentage of used gas by \pri \txs, which also relate to the first abnormal period in~\secref{sec:char:dis}.
    For another example, block 14,520,420 has only one \tx and this \tx is a \pri \tx. 
    Besides, there are 367 blocks in total whose used gas percentage by \pri \txs is 100\%. In addition, 361 blocks are mined after the gas limit expansion and 6 blocks are before the expansion. 
    
    From the above experiments, we observe that the expansion of the gas limit helps the growth of \pri \txs. Before the gas limit expansion in block 12,965,000, the used gas by total \txs is about 99\% of the gas limit on average. It shows that the Ethereum network is somehow crowded and \txs are awaiting to be mined. Besides, after the gas limit is increased, miners have the abilities of packing more \txs. Accordingly, the number of \pri \txs in blocks can be dynamically increased. After the gas limit is increased, the average ratio of gas used by each block to its gas limit drops to about 63\%. \xz{this is about total tx, not private tx}
    
    \lesson{The used gas by \pri \txs on average is about 780,000 \textit{GWei} and takes 5.8\% among the total.}
    
    % \mz{@xingyu, double check, what does the gas limitation expansion mean?}\xl{In the Ethereum network, there is an upper limit on how many transaction instructions each block can process, namely the Block Gas Limit. After EIP-1559, the gas limit of block gas was increased according to the network transaction demand. The average block gas upper limit in a period of time remains unchanged, it can  avoid network congestion caused by it.}
    
    % The gas used in each \tx reflects the computation power needed to deal with it. 
    % Previously, the MEV congestion happened in the mainnet \cite{???} due to the large amount of usedgas. 
    % From the figure~\figref{figs:usedgas}, the \pri \txs only take a small portion of total \txs. Besides, the maximum percentage of used gas is xxx\% in block xxx. 
    % Thus, the current \pri \txs cannot congest the network due to the powerful computation, such as DoS attack. 

\subsection {Categories} 
\label{sec:eval:category}
\xz{this subsection can be merged with 4.1}
    The \pri \txs can be categorised into four types with regarding of their usages and purposes, as follows.
    \xz{why are we making the categorization? what are the benefits/goals?}
    \begin{packeditemize}
        \item Type I: the \pri \txs that MEV Bots participate in. \Pri \txs of this type should have MEVBots as their recipients and are usually used for MEV extraction.
        \item Type II: the \pri \txs used to transfer money to EOAs. \Pri \txs of this type are normally sent from miners or other well-known services and used to transfer \textit{ETH}.
        %\mz{@xingyu, the receivers of Type II can be smart contracts? pls check the correctness}
        % and have EOAs as receivers. In addition, such \txs also include transferring money through smart contracts.
        \item Type III: the \pri \txs that are only used for DeFi services (e.g. Uniswap trader).
        % This type of privacy transaction is usually to protect its own transactions to avoid some risks brought in the public mempool. \mz{@xingyu, I think you cannot prove this, how do you know their intentions?} 
        % @\mz{@xingyu, the usage does not match the example. So this type is not only used for avoiding MEV risks? They are just calling DeFi services?}
        % usually to protect their own transactions from attacks such as front-running, and avoid the risks brought by MEV. For example, traders in Uniswap are only to exchange the corresponding token. 
        \item Type IV: the remaining \pri \txs whose  receivers are normal smart contract that cannot be labeled.
        These \pri \txs aim to have a higher success rate of being mined into the block. %\mz{unclear on the purposes}
        % senders are not miners and receivers are usually ordinary smart contract addresses without labels. These transactions complete specific transaction logic through the privacy properties , such as arbitrage through smart contracts, etc.
    \end{packeditemize}
    
    % \bheading{Methods to categorize the three types.} 
    % Basically, the types of \pri \txs are classified based on the senders and receivers. \mz{@all, not sure this is reasonable.} \mz{@xingyu, can you double check the methods? } \mz{rewrite}
    % \begin{itemize}
    %     \item Type I: the receivers of the \txs should be MEVBots.
    %     % \item Type II: the receivers of the \txs are smart contracts, but not MEVBots. Besides, the senders should not be miners. 
    %     % \item Type III: the senders of the \txs should be miners and the receivers should not be MEVBots.
    %     % \item Type I: the money flow shows the sign of arbitrage and the arbitrager is not necessarily able to make money. 
    %     % \item Type II: the smart contracts called in such \txs are usually the DeFi platforms and the functions are generally services provided by DeFi. Besides, these \txs are non-profitable. 
    %     % \item Type III: the senders of these \txs are miners and only have simple token transfers in the money flow. Specifically, the transferre token is always ETH.  
    % \end{itemize}
    
    \bheading{The statistics of four types of \pri \txs.}
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/42ptxs/42_px_type.pdf}
    \caption{The count of \pri \txs in each type by per month(x: the count of \pri \txs in each type; y: per type per month).}
    \label{figs:typepermonth}
    \end{figure}
    We present the count of \pri \txs of each type against per month in ~\figref{figs:typepermonth}. 
    For type I, there are 28.6\% of \pri \txs that are sent to MEV Bots, which shows the increasing need of \pri \txs for MEV searchers since the competition of MEV becomes more and more fierce.
    For type II, 22.4\% of \pri \txs are used for transfers. In particular, the senders of these \pri \txs are miners and well-known services(e.g., Crypto.com~\cite{crypto}).  
    For type III, about 18.1\% of \pri \txs are sent to call DeFi related services. 
    Besides, the left 30.9\% of \pri \txs belong to type IV. Among them, about 650,000 transactions are used for transferring tokens through the smart contracts. 
    \xz{do we have more about MEV in later section?}
    % \mz{@all, should we keep this subsection?}
    
    \lesson{We categorize the \pri \txs into four types. Specifically, the type I that involves in MEVBots takes 28.6\% and the type II transferring \textit{ETH} from miners accounts for 22.4\%.}


\subsection{Tokens and DeFi Platforms}
    \subsubsection{The top tokens used in \pri \txs, the patterns of tokens, and the distributions.} In this part, we measure the top tokens initially used and lastly owned in the \pri \txs. \xz{again, why we care about this? explain} Besides, we classify the token patterns in \pri \txs into five categories and quantify the distributions of these types.
    % \mz{@xingyu, use heatmap to show the data and re-explain the data in paper}
    % \bheading{The top type of tokens initially used in the \pri \txs.}
    % We utilize the information of token flows extracted before and measure the top initially used tokens in \pri \txs.
    % The top 1 ERC20 tokens initially used are mostly \textit{WETH} that is the representation of \textit{ETH} in ERC20 implementation, according to ~\figref{figs:initialtoken}. Then, the most frequently used tokens are basically stablecoins, such as the top 2 token USDC and the top 3 token Tether.
    
    % \bheading{The top type of tokens lastly owned in the \pri \txs.} 
    % We measure the top type of tokens by extracting all the token transfers in the money flow and obtain the last token types with amounts in the \pri \txs. 
    % As displayed in ~\figref{figs:lasttoken}, the lastly owned token types are basically same as the initially used token types. Besides, these tokens are mostly either \textit{WETH} or the stablecoins. 

    \bheading{The top tokens initially used and lastly owned pairs in the \pri \txs.}
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/43ptxs/43_top_token_pairs_2.pdf}
    \caption{The top type of tokens initially used and lastly owned in the \pri \txs.} 
    \label{figs:token-pairs}
    \end{figure}
    From ~\figref{figs:token-pairs}, the top 2 token pairs are (\textit{ETH}, \textit{USDC}) and (\textit{USDC}, \textit{ETH}). In particular, the count of top 1 token pair \textit{ETH}, \textit{USDC}) is xxx, accounting for xxx\% in the total pairs. For the rest of the top token pairs, they are all either \textit{ETH} or stablecoins.xxx \mz{@xingyu, explain here, write 2-3 sentences} \mz{check correctness, any token is not stablecoin here?}
    
    \lesson{The most used tokens initially and lastly owned are either \textit{ETH} or stablecoins.}
    
    
    \bheading{The token swap patterns.}
    We classify the token swap patterns in the \pri \txs into the following five types.
    \xz{again, why are we perform the classification here?}
    \begin{packeditemize}
        \item Type I: a simple transfer.
        \item Type II: involving in two types of tokens and two token transfer edges.
        \item Type III: involving in two types of tokens but more than two token transfer edges.
        \item Type IV: involving in three types of tokens.
        \item Type V: involving in  more than three types of token.
    \end{packeditemize}
    % \begin{figure}[t]
    % \centering
    % \includegraphics[width=1\columnwidth]{figs/431_The token swap patterns used in the px.png}
    % \caption{The count of \pri \txs in each token swap pattern(x: the count of \pri \txs; y: each type).}
    % \label{figs:swappattern}
    % \end{figure}

    \begin{table}[h]
    \centering
    \begin{tabular}{l | l | l | l| l}
    Type I & Type II  & Type III & Type IV &  Type V \\
    \hline
    12.80\% & 50.50\%& 18.90\% & 15.60\% & 2.2\%
    \end{tabular}
    \caption{very basic table}
    \label{tab:abc}
    \end{table} 

    % \mz{@xingyu, revise the figure since I modified the types in paper(simple -> complex type), check paper.} done
    \tabref{tab:abc} shows the count of \pri \txs against each token swap type. 
    Specifically, the exchange between two tokens that the type II and type III accounts for about 69\% of among all token swap \txs, which is the largest part. This \txs mode usually occurs in one or two AMM ~\mz{cite and explain AMM here, one sentence} services. \mz{@xingyu, we can use table, but revise it}
    
    \lesson{Around 69\% \pri \txs involve in two types of tokens in the money flow.}
    
    
    \bheading{The top 10 token exchange pairs in \pri \txs.}
    %  \begin{figure}[t]
    % \centering
    % \includegraphics[width=1\columnwidth]{figs/431_The top token exchange pairs in private transactions.png}
    % \caption{The top 10 token exchange pairs in \pri \txs(x: the count of the token pairs; y: the token pair).}
    % \label{figs:pairs}
    % \end{figure}
    We measure the mostly often used token exchange pairs of the \pri \txs in ~\figref{figs:pairs}. From the figure, we observe that the exchanges between \textit{ETH} and the stablecoin \textit{USDC} are the top 2 token pairs. Besides, all the top 10 exchange pairs contain \textit{ETH} token and the rest token types mainly are stablecoins. \mz{compare the last two figures and explain the differences.}
    
    \lesson{The top 10 token exchange pairs are mainly \textit{WETH} and stablecoins.}
    
\subsubsection{The top DeFi services and platforms used by \pri \txs.} 
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/43ptxs/43_defi_top.pdf}
    \caption{The 10 top DeFi platforms involved in \pri \txs.}
    \label{figs:defi}
    \end{figure}
    
    % By analyzing the privacy transactions between users and DeFi services, we found that more than 60\% of the transaction privacy transactions are mainly involved in the token transactions of AMM exchanges. The most popular ones are Uniswap V2, Uniswap V3, SushiSwap, etc. These service providers use the corresponding economic The model guarantees the liquidity of tokens, and the initiators of private transactions can obtain MEV opportunities from these DeFi services. For example, searchers can obtain the price slippage of the same token on different exchanges to arbitrage. In addition, 61,740 transactions were identified using OpenSea services. OpenSea is an NFT-based decentralized market for trading rare digital goods running on Ethereum, which is closely related to the popularity of the NFT market.
    We present the count of \pri \txs against the DeFi platform in the top 10. More than 60\% of the \pri \txs are AMM exchanges and the related mostly used top three DeFi platforms are Uniswap V2~\cite{}, Uniswap V3~\cite{}, and SushiSwap~\cite{}. \xz{use a different font type for platforms/tokens} Those \pri \txs target at these platforms to search for MEV opportunities. For example, MEV searchers can utilize the price slippage of the same token on different platforms to make money. 
    In addition, 61,740 \pri \txs are identified using OpenSea~\cite{} platform that is an None Fungible Token (NFT) based decentralized market for trading rare digital goods running on Ethereum.
    
    \lesson{Most \pri \txs use DeFi platforms for MEV opportunities and NFT platform for trading.}
   
    % As expected, platform Uniswap~\cite{} is the most used platform among the \pri \txs since it is the largest ??? DEX in Ethereum blockchain. 
  
    % Among the services used by privacy exchanges, more than 60 \% of the transactions focus on AMMs about token exchanges, the most popular ones are Uniswap (V2/V3), SushiSwap, 1inch (V3/V4), etc., all of which are exchanges It is a decentralized exchange that automates market makers and replaces manual quotations with established algorithms. Based on the "constant product automatic market making" model [reserve pool mode, on-chain matching, on-chain clearing], and promotes ETH and ERC20 Automatic exchange transaction between token digital assets

    % In addition, 61,740 transactions were identified using the services of OpenSea, a decentralized peer-to-peer marketplace for buying, selling and trading rare digital goods, from game items to collectibles to art, built on irreplaceable on top of the Token (NFT) technology and runs on the Ethereum blockchain.
  
    
\subsubsection{The tokens used among the top services and platforms in \pri \txs.} 
     In this paper, we summarize the services used in privacy transactions into two categories: one is traditional AMM, represented by uniswap and sushiswap; the other is a trading platform for digital assets such as artworks, which is represented by uniswap and sushiswap. Opensea is the representative. Therefore, in this section, we will analyze the transactions on the traditional AMM Uniswap Router and the new trading platform opensea, and analyze the tokens and token swap modes used by these two services, which can better help us understand private transactions.
        
    In uniswap-related privacy transactions (including uniswap V2, V3), the most used tokens at the beginning and the first three tokens held at the end are ETH, USDC, and USDT stable coins, with a ratio of more than 40\%. There are 555,643 transactions of the two types of tokens in uniswap the most common, of which about 41\% are transactions of other tokens converted into stable coins,
        
        \xz{is this a case study?}
    In the opensea transaction, the top three tokens held at the beginning are ETH, CryptoZoo Base Egg (EGG), Art Blocks (BLOCKS), and the top three tokens held last are CryptoZoo Base Egg (EGG), Art Blocks (BLOCKS), ETH, of which CryptoZoo Base Egg (EGG), Art Blocks (BLOCKS) belong to ERC-721 Token. The most transactions of Opesea are transfers between the two through the smart contract, which accounts for more than 50\% of the total transactions of Opensea. The behavior of this part of the transaction is that after the user purchases NFT assets in opensea, the NFT is transferred from the original owner to the current buyer, and the seller will receive income from opensea.The most commonly used token for purchasing NFT is CryptoZoo Base Egg (EGG), which accounts for 24\% of the total transactions. \mz{@xingyu, please give the top exchange pairs for uniswap and opensea.}\xl{The most popular tx pattern in opensea is: A -> NFT->B,B->Token->A,so no exchange pairs; uniswap's pairs is similar as top 10 pairs(top 5 are the same),so I want to conclud its pairs as other tokens -> stablecoins }
    
    \lesson{}
        
    
\subsection{Arbitrage Detection}
\xz{need some transitions to this arbitrage subsection; also need to highlight why we detect arbitrage and why it is important. Maybe we can refer to the BEV paper (SP'22) on the arbitrage detection data}
We define two types of arbitrages: cyclic arbitrage and nonce-cyclic arbitrage, introduce the detection algorithms, and measures the detection accuracy in~\appref{sec:arbitrage}. Here we analyze the detected results of the \pri \txs as follows. 

    \bheading{Top Arbitraguers.}
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/44ptxs/4_arbitrage_type.pdf}
    % \vspace*{-9mm}
    \caption{The type of arbitrage in \pri \txs .}
    \label{figs:trec}
    \end{figure}
    
    \bheading{Top Arbitraguers.}
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/44ptxs/4_top_10_arbritrage.pdf}
    % \vspace*{-9mm}
    \caption{The type of arbitrage in \pri \txs .}
    \label{figs:trec}
    \end{figure}
    
    Summary: there are xxx \pri \txs flagged as arbitrage. Specifically, there are 376393 of them belonging to Type I and 722613 of them for Type II. 
    
    
    \bheading{Profit of the arbitrage \txs}
    
    \bheading{Top Arbitraguers.}
    \begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figs/44ptxs/4_total_profit.pdf}
    % \vspace*{-9mm}
    \caption{The type of arbitrage in \pri \txs .}
    \label{figs:trec}
    \end{figure}
    
    
    \bheading{Position of the arbitrage \txs in blocks}
    
    About 97\% of the private transactions containing Arbitrage are in the top ten of the block. In addition, about 3\% of the transactions are located after the tenth position of the block. These blocks contain a large number of transactions. In addition, the top of these blocks usually contains the miner's transfer to the EOA address.
    
    
    \pri \txs needs to ensure an earlier position in order to obtain the opportunity to be on the chain as soon as possible to realize operations such as token exchange. 
    
    \bheading{Token swap types of arbitrage \txs} 
    
    
    
    
    \lesson{}


